OTTER: One-Step Teacher-Free Image Restoration via Nonparametric Score Distillation

Conventional score distillation provides distribution-level supervision for one-step diffusion restoration but typically requires a Teacher Model and an Auxiliary Network. Drifting removes the Auxiliary Network by estimating supervision directly from sample sets. However, deterministic paired restoration provides only one high-quality target and one student output per input, a limitation we term conditional sample collapse. We address this limitation through OTTER, which introduces Nonparametric Score Distillation as a teacher-free, task- and backbone-agnostic training objective for paired image restoration. Our central insight is that spatial recurrence within a single image pair supplies internal surrogate samples for attraction and repulsion. We construct these sample sets from recurring high-quality residuals and corresponding student residuals relative to the low-quality input. Attraction weights computed solely from high-quality residuals reduce sensitivity to student errors. Regression toward the drifted target operates on the high-frequency band of decoded images, while paired reconstruction losses preserve fidelity. In the diffusion setting, OTTER trains with a single diffusion-scale network forward pass per iteration, without a Teacher Model, Auxiliary Network, Discriminator, or alternating optimization. Experiments on real-world image super-resolution and all-in-one image restoration demonstrate improved fidelity and perceptual similarity with U-Net, diffusion transformer, and Restormer backbones.

==> otter-style.tex <==
% arxiv2027/otter-style.tex

% Ubuntu for the title panel and numbered main-paper sections.
\RequirePackage{iftex}
\ifXeTeX
\DeclareFontFamily{TU}{otterubuntu}{}
\DeclareFontShape{TU}{otterubuntu}{m}{n}
  {<-> "[\OtterArchiveRoot assets/ubuntu/Ubuntu-Regular.ttf]:mapping=tex-text"}{}
\DeclareFontShape{TU}{otterubuntu}{b}{n}
  {<-> "[\OtterArchiveRoot assets/ubuntu/Ubuntu-Medium.ttf]:mapping=tex-text"}{}

\newcommand{\UbuntuTitle}{\usefont{TU}{otterubuntu}{m}{n}}
\newcommand{\OtterMainSectionFace}{\usefont{TU}{otterubuntu}{b}{n}}
\newcommand{\UbuntuHeading}{\bfseries}

% Support curly apostrophes in the OT1 Times body text.
\catcode`’=\active
\protected\def’{\textquoteright}

\else
  % Keep the Overleaf TPAMI project's default pdfLaTeX compiler unchanged.
  \newcommand{\UbuntuTitle}{\fontfamily{phv}\fontseries{m}\selectfont}
  \newcommand{\OtterMainSectionFace}{\fontfamily{phv}\fontseries{b}\selectfont}
  \newcommand{\UbuntuHeading}{\bfseries}
  \DeclareUnicodeCharacter{2019}{\textquoteright}
\fi

\definecolor{TitleInk}{HTML}{10217C}
\definecolor{TitlePanel}{HTML}{F3F5FA}
\hypersetup{bookmarksnumbered=true,pdfdisplaydoctitle=true}

% Main-paper section headings.
\let\RestoreCVPRSectionFormat\cvprsection
\newcommand{\UseMainSectionFont}{%
  \patchcmd{\cvprsection}
    {\large\bf}
    {\large\OtterMainSectionFace}
    {}
    {\PackageError{otter}{Could not apply the main section font}
       {Check the section definition in cvpr.sty.}}%
}
\newcommand{\RestoreCVPRSectionFont}{%
  \let\cvprsection\RestoreCVPRSectionFormat
}

\newcommand{\OtterAuthor}[2]{%
  \mbox{#1\textsuperscript{#2}}%
}

\renewcommand{\maketitle}{%
  \begin{tcolorbox}[
    colback=TitlePanel,
    colframe=TitlePanel,
    boxrule=0pt,
    arc=9pt,
    outer arc=9pt,
    boxsep=0pt,
    left=12pt,
    right=12pt,
    top=8pt,
    bottom=6pt,
    before skip=0pt,
    after skip=8pt
  ]
    \centering

    % Paper title
    {\UbuntuTitle\fontsize{14.1}{16.2}\selectfont
      \color{TitleInk}\PaperTitleLines{\\}\par}

    \vspace{6pt}

    % Authors
    {\UbuntuTitle\fontsize{9.3}{11}\selectfont
      \OtterAuthor{Seungho Choi}{1}\quad
      \OtterAuthor{Sanglim Han}{1}\quad
      \OtterAuthor{Victoria Vesna}{2}\quad
      \OtterAuthor{Jihyong Oh}{1,\textdagger}\par}

    \vspace{1pt}

    % Left: OTTER icon
    \noindent
    \begin{minipage}[c]{.19\linewidth}
      \centering
      \includegraphics[width=54pt]{\OtterArchiveRoot assets/otter.png}
    \end{minipage}\hfill
    % Center: affiliations and contact information
    \begin{minipage}[c]{.56\linewidth}
      \centering
      \fontsize{8.7}{10.3}\selectfont
      \begin{tabular}{@{}c@{\hspace{13pt}}c@{}}
        \textsuperscript{1}\,CMLab, Chung-Ang University &
        \textsuperscript{2}\,UCLA\\[2pt]
        {\fontsize{7.3}{8.7}\selectfont
          (\{choiseungho1019, sanglimhan, jihyongoh\}@cau.ac.kr)} &
        {\fontsize{7.3}{8.7}\selectfont
          (vesna@arts.ucla.edu)}
      \end{tabular}
    \end{minipage}\hfill
    % Right: institution logos
    \begin{minipage}[c]{.19\linewidth}
      \centering
      \href{https://cmlab-korea.github.io/}{\includegraphics[width=68pt]{\OtterArchiveRoot assets/cmlab.png}}\\[6pt]
      \includegraphics[height=22pt]{\OtterArchiveRoot assets/ucla-wordmark.pdf}
    \end{minipage}\par

    \vspace{2pt}
    {\fontsize{7.3}{8.7}\selectfont \textsuperscript{\textdagger}Corresponding author\par}

    % Project page, centered at the bottom of the title panel
    \vspace{4pt}
    {\centering
      \fontsize{8}{9.5}\selectfont
      \color{TitleInk}%
      \ifdefvoid{\ProjectPageURL}
        {\def\OtterURL{https://cmlab-korea.github.io/OTTER/}}
        {\let\OtterURL\ProjectPageURL}%
      \hypersetup{urlcolor=TitleInk}%
      \urlstyle{tt}%
      \textbf{Project page:}\enspace
      \expandafter\url\expandafter{\OtterURL}\par}

  \end{tcolorbox}%
}

\AddToHook{bfseries}{\OtterMainSectionFace}
\renewcommand*{\elvbf}{\fontsize{11}{13.2}\OtterMainSectionFace}

\DeclareCaptionFont{ottermedium}{\OtterMainSectionFace}

\captionsetup[figure]{labelfont=ottermedium}
\captionsetup[table]{labelfont=ottermedium}
